Prompting Large Vision-Language Models for Compositional Reasoning

Vision-language models such as CLIP have shown impressive capabilities in encoding texts and images into aligned embeddings, enabling the retrieval of multimodal data in a shared embedding space. However, these embedding-based models still face challenges in effectively matching images and texts with similar visio-linguistic compositionality, as evidenced by their performance on the recent Winoground dataset. In this paper, we argue that this limitation stems from two factors: the use of single vector representations for complex multimodal data, and the absence of step-by-step reasoning in these embedding-based methods. To address this issue, we make an exploratory step using a novel generative method that prompts large vision-language models (e.g., GPT-4) to depict images and perform compositional reasoning. Our method outperforms other embedding-based methods on the Winoground dataset, and obtains further improvement of up to 10% accuracy when enhanced with the optimal description.

==> tables/fine_grained.tex <==
\begin{table*}[h]
    \centering
    \toprule[1pt]
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c}
        Method & Non-Compositional & Ambiguously Correct & Visually Difficult & Unusual Image & Unusual Text & Complex Reasoning & No Tag \\

        % 50.98	32.22333333	48.33333333	15.83333333	16.27666667	28.63333333	31.59333333
        Ours & 52.94 &  34.45 & 31.67 & 34.17 & 26.36 & 32.91 & 39.53  \\
        Ours (No Keywords) & 37.25 &  20.00 & 20 & 16.67 & 21.70 & 17.09 & 23.64  \\
        Ours (No Explanation) & 50.98 &  32.22 & 48.33 & 15.83 & 16.28 & 28.63 & 31.59  \\


        MiniGPT4 Only & 18.89 &  18.84 & 0 & 22.02 & 18.67 & 10.26 & 17.93  \\
        \midrule

        CLIP  & 76.6 &  30.43 & 15.79 & 25 & 30 & 24.36 & 30.41  \\
 
        
    \end{tabular}
    }
    \bottomrule[1pt]
    \caption{\small Average performance on individual question categories for the Winoground task. Our method shows significant improvement on complex reasoning questions, which make up a large portion of the dataset.}
    \label{tab:fine_grained}
\end{table*}
